Etale Fundamental group of moduli of torsors under Bruhat-Tits group scheme over a curve

Let $X$ be a smooth projective curve over an algebraically closed field $k$. Let $\mathcal{G}$ be a Bruhat-Tits group scheme on $X$ which is generically semi-simple and trivial. We show that the \'etale fundamental group of the moduli stack $\mathcal{M}_X(\mathcal{G})$ of torsors under $\mathcal{G}$ is isomorphic to that of the moduli stack $\mathcal{M}_X(G)$ of principal $G$-bundles. For any smooth, noetherian and irreducible stack $\mathcal{X}$, we show that an inclusion of an open substack $\mathcal{X}^\circ$, whose complement has codimension at least two, will induce an isomorphism of \'etale fundamental group. Over $\mathbb{C}$, we show that the open substack of regularly stable torsors in $\mathcal{M}_X(\mathcal{G})$ has complement of codimension at least two when $g_X \geq 3$. As an application, we show that the moduli space $M_X(\mathcal{G})$ of $\mathcal{G}$-torsors is simply-connected.

==> fourier.tex <==
\def\fileversion{1.4}%
\def\filedate{2005/01/01}%
\NeedsTeXFormat{LaTeX2e}%
\ProvidesPackage{fourier}%
[\filedate\space\fileversion\space fourier-GUTenberg package]%
\DeclareFontEncoding{FML}{}{}
  \DeclareFontSubstitution{FML}{futm}{m}{it}
\DeclareFontEncoding{FMS}{}{}
  \DeclareFontSubstitution{FMS}{futm}{m}{n}
\DeclareFontEncoding{FMX}{}{}
  \DeclareFontSubstitution{FMX}{futm}{m}{n}
%%
\newif\ifsloped\newif\ifpoorman\poormantrue
\newif\ifwidespace\widespacefalse
\DeclareOption{widespace}{\widespacetrue}
%%
\DeclareOption{poorman}{\def\textfamilyextension{s}%
\def\mathfamilyextension{s}}
\DeclareOption{expert}{\def\textfamilyextension{x}%
\def\mathfamilyextension{x}\poormanfalse}
\DeclareOption{oldstyle}{\def\textfamilyextension{j}%
\def\mathfamilyextension{x}\poormanfalse}
\DeclareOption{fulloldstyle}{\def\textfamilyextension{j}%
\def\mathfamilyextension{j}\poormanfalse}
\DeclareOption{sloped}{\slopedtrue}
\DeclareOption{upright}{\slopedfalse}
\ExecuteOptions{sloped,poorman}
\ProcessOptions
%%

%%
\ifwidespace
\DeclareRobustCommand{\SetFourierSpace}{%
\fontdimen2\font=1.23\fontdimen2\font}
\fi
\ifpoorman\else
\newcommand*{\sbseries}{\fontseries{sb}\selectfont}
\newcommand*{\blackseries}{\fontseries{eb}\selectfont}
\newcommand*{\titleshape}{\fontshape{tt}\selectfont}
\DeclareTextFontCommand{\textsb}{\sbseries}%
\DeclareTextFontCommand{\textblack}{\blackseries}%
\DeclareTextFontCommand{\texttitle}{\titleshape}%
\newcommand*{\oldstyle}{\fontfamily{futj}\selectfont}
\newcommand*{\lining}{\fontfamily{futx}\selectfont}
\fi
\renewcommand{\rmdefault}{fut\textfamilyextension}
\RequirePackage[T1]{fontenc}
\RequirePackage{textcomp}
\RequirePackage{fourier-orns}
\DeclareSymbolFont{operators}{T1}{fut\mathfamilyextension}{m}{n}%
\SetSymbolFont{operators}{bold}{T1}{fut\mathfamilyextension}{b}{n}%

%
\def\addFourierGreekPrefix#1{other}
\newcommand{\othergreek}[1]{\expandafter\csname\expandafter%
\addFourierGreekPrefix\string#1\endcsname}
%
\ifsloped
\DeclareSymbolFont{letters}{FML}{futmi}{m}{it}%
\DeclareSymbolFont{otherletters}{FML}{futm}{m}{it}
\SetSymbolFont{letters}{bold}{FML}{futmi}{b}{it}
\SetSymbolFont{otherletters}{bold}{FML}{futm}{b}{it}
\DeclareMathSymbol{\Gamma}{\mathord}{otherletters}{000}
\DeclareMathSymbol{\Delta}{\mathord}{otherletters}{001}
\DeclareMathSymbol{\Theta}{\mathord}{otherletters}{002}
\DeclareMathSymbol{\Lambda}{\mathord}{otherletters}{003}
\DeclareMathSymbol{\Xi}{\mathord}{otherletters}{004}
\DeclareMathSymbol{\Pi}{\mathord}{otherletters}{005}
\DeclareMathSymbol{\Sigma}{\mathord}{otherletters}{006}
\DeclareMathSymbol{\Upsilon}{\mathord}{otherletters}{007}
\DeclareMathSymbol{\Phi}{\mathord}{otherletters}{008}
\DeclareMathSymbol{\Psi}{\mathord}{otherletters}{009}
\DeclareMathSymbol{\Omega}{\mathord}{otherletters}{010}
\DeclareMathSymbol{\otherGamma}{\mathord}{letters}{000}
\DeclareMathSymbol{\otherDelta}{\mathord}{letters}{001}
\DeclareMathSymbol{\otherTheta}{\mathord}{letters}{002}
\DeclareMathSymbol{\otherLambda}{\mathord}{letters}{003}
\DeclareMathSymbol{\otherXi}{\mathord}{letters}{004}
\DeclareMathSymbol{\otherPi}{\mathord}{letters}{005}
\DeclareMathSymbol{\otherSigma}{\mathord}{letters}{006}
\DeclareMathSymbol{\otherUpsilon}{\mathord}{letters}{007}
\DeclareMathSymbol{\otherPhi}{\mathord}{letters}{008}
\DeclareMathSymbol{\otherPsi}{\mathord}{letters}{009}
\DeclareMathSymbol{\otherOmega}{\mathord}{letters}{010}
\else
\DeclareSymbolFont{letters}{FML}{futm}{m}{it}%
\DeclareSymbolFont{otherletters}{FML}{futmi}{m}{it}
\SetSymbolFont{letters}{bold}{FML}{futm}{b}{it}
\SetSymbolFont{otherletters}{bold}{FML}{futmi}{b}{it}
\DeclareMathSymbol{\Gamma}{\mathord}{letters}{000}
\DeclareMathSymbol{\Delta}{\mathord}{letters}{001}
\DeclareMathSymbol{\Theta}{\mathord}{letters}{002}
\DeclareMathSymbol{\Lambda}{\mathord}{letters}{003}
\DeclareMathSymbol{\Xi}{\mathord}{letters}{004}
\DeclareMathSymbol{\Pi}{\mathord}{letters}{005}
\DeclareMathSymbol{\Sigma}{\mathord}{letters}{006}
\DeclareMathSymbol{\Upsilon}{\mathord}{letters}{007}
\DeclareMathSymbol{\Phi}{\mathord}{letters}{008}
\DeclareMathSymbol{\Psi}{\mathord}{letters}{009}
\DeclareMathSymbol{\Omega}{\mathord}{letters}{010}
\DeclareMathSymbol{\otherGamma}{\mathord}{otherletters}{000}
\DeclareMathSymbol{\otherDelta}{\mathord}{otherletters}{001}
\DeclareMathSymbol{\otherTheta}{\mathord}{otherletters}{002}
\DeclareMathSymbol{\otherLambda}{\mathord}{otherletters}{003}
\DeclareMathSymbol{\otherXi}{\mathord}{otherletters}{004}
\DeclareMathSymbol{\otherPi}{\mathord}{otherletters}{005}
\DeclareMathSymbol{\otherSigma}{\mathord}{otherletters}{006}
\DeclareMathSymbol{\otherUpsilon}{\mathord}{otherletters}{007}
\DeclareMathSymbol{\otherPhi}{\mathord}{otherletters}{008}
\DeclareMathSymbol{\otherPsi}{\mathord}{otherletters}{009}
\DeclareMathSymbol{\otherOmega}{\mathord}{otherletters}{010}
\fi
\DeclareSymbolFont{symbols}{FMS}{futm}{m}{n}%
\DeclareSymbolFont{largesymbols}{FMX}{futm}{m}{n}
\DeclareMathAlphabet{\mathbf}{T1}{fut\mathfamilyextension}{bx}{n}%
\DeclareMathAlphabet{\mathrm}{T1}{fut\mathfamilyextension}{m}{n}%
\DeclareMathAlphabet{\mathit}{T1}{fut\mathfamilyextension}{m}{it}%
\DeclareMathAlphabet{\mathcal}{FMS}{futm}{m}{n}%
\DeclareMathSymbol{\varkappa}{\mathord}{letters}{128}
\DeclareMathSymbol{\varvarrho}{\mathord}{letters}{129}
\DeclareMathSymbol{+}{\mathbin}{symbols}{128}
\DeclareMathSymbol{=}{\mathrel}{symbols}{129}
\DeclareMathSymbol{<}{\mathrel}{symbols}{130}
\DeclareMathSymbol{>}{\mathrel}{symbols}{131}
\DeclareMathSymbol{\leqslant}{\mathrel}{symbols}{132}
\DeclareMathSymbol{\geqslant}{\mathrel}{symbols}{133}
\DeclareMathSymbol{\parallelslant}{\mathrel}{symbols}{134}
\DeclareMathSymbol{\thething}{\mathord}{symbols}{135}
\DeclareMathSymbol{\vDash}{\mathrel}{symbols}{136}
\DeclareMathSymbol{\blacktriangleleft}{\mathrel}{symbols}{137}
\DeclareMathSymbol{\blacktriangleright}{\mathrel}{symbols}{138}
\DeclareMathSymbol{\nleqslant}{\mathrel}{symbols}{139}
\DeclareMathSymbol{\ngeqslant}{\mathrel}{symbols}{140}
\DeclareMathSymbol{\parallel}{\mathrel}{symbols}{141}
\DeclareMathSymbol{\nparallel}{\mathrel}{symbols}{142}
\DeclareMathSymbol{\nparallelslant}{\mathrel}{symbols}{143}
\DeclareMathSymbol{\nvDash}{\mathrel}{symbols}{144}
\DeclareMathSymbol{\intercal}{\mathbin}{symbols}{145}
\DeclareMathSymbol{\hslash}{\mathord}{symbols}{146}
\DeclareMathSymbol{\nexists}{\mathord}{symbols}{147}
\DeclareMathSymbol{\complement}{\mathord}{symbols}{148}
\DeclareMathSymbol{\varsubsetneq}{\mathrel}{symbols}{149}
\DeclareMathSymbol{\xswordsup}{\mathord}{symbols}{150}
\DeclareMathSymbol{\xswordsdown}{\mathord}{symbols}{151}
\let\notin\@undefined
\DeclareMathSymbol{\notin}{\mathrel}{symbols}{155}
\DeclareMathSymbol{\notowns}{\mathrel}{symbols}{156}
\DeclareMathSymbol{\hbar}{\mathord}{symbols}{157}
\DeclareMathSymbol{\smallsetminus}{\mathbin}{symbols}{158}
\DeclareMathSymbol{\subsetneqq}{\mathrel}{symbols}{159}
\DeclareMathSymbol{\rightrightarrows}{\mathrel}{symbols}{160}
\DeclareMathSymbol{\leftleftarrows}{\mathrel}{symbols}{161}
\DeclareMathSymbol{\square}{\mathord}{symbols}{162}
\DeclareMathSymbol{\curvearrowleft}{\mathrel}{symbols}{163}
\DeclareMathSymbol{\curvearrowright}{\mathrel}{symbols}{164}
\DeclareMathSymbol{\blacksquare}{\mathord}{symbols}{165}
\DeclareMathSymbol{\otheralpha}{\mathord}{otherletters}{011}
\DeclareMathSymbol{\otherbeta}{\mathord}{otherletters}{012}
\DeclareMathSymbol{\othergamma}{\mathord}{otherletters}{013}
\DeclareMathSymbol{\otherdelta}{\mathord}{otherletters}{014}
\DeclareMathSymbol{\otherepsilon}{\mathord}{otherletters}{015}
\DeclareMathSymbol{\otherzeta}{\mathord}{otherletters}{016}
\DeclareMathSymbol{\othereta}{\mathord}{otherletters}{017}
\DeclareMathSymbol{\othertheta}{\mathord}{otherletters}{018}
\DeclareMathSymbol{\otheriota}{\mathord}{otherletters}{019}
\DeclareMathSymbol{\otherkappa}{\mathord}{otherletters}{020}
\DeclareMathSymbol{\otherlambda}{\mathord}{otherletters}{021}
\DeclareMathSymbol{\othermu}{\mathord}{otherletters}{022}
\DeclareMathSymbol{\othernu}{\mathord}{otherletters}{023}
\DeclareMathSymbol{\otherxi}{\mathord}{otherletters}{024}
\DeclareMathSymbol{\otherpi}{\mathord}{otherletters}{025}
\DeclareMathSymbol{\otherrho}{\mathord}{otherletters}{026}
\DeclareMathSymbol{\othersigma}{\mathord}{otherletters}{027}
\DeclareMathSymbol{\othertau}{\mathord}{otherletters}{028}
\DeclareMathSymbol{\otherupsilon}{\mathord}{otherletters}{029}
\DeclareMathSymbol{\otherphi}{\mathord}{otherletters}{030}
\DeclareMathSymbol{\otherchi}{\mathord}{otherletters}{031}
\DeclareMathSymbol{\otherpsi}{\mathord}{otherletters}{032}
\DeclareMathSymbol{\otheromega}{\mathord}{otherletters}{033}
\DeclareMathSymbol{\othervarepsilon}{\mathord}{otherletters}{034}
\DeclareMathSymbol{\othervartheta}{\mathord}{otherletters}{035}
\DeclareMathSymbol{\othervarpi}{\mathord}{otherletters}{036}
\DeclareMathSymbol{\othervarrho}{\mathord}{otherletters}{037}
\DeclareMathSymbol{\othervarsigma}{\mathord}{otherletters}{038}
\DeclareMathSymbol{\othervarphi}{\mathord}{otherletters}{039}
\DeclareMathSymbol{\varkappa}{\mathord}{letters}{128}
\DeclareMathSymbol{\varvarrho}{\mathord}{letters}{129}
\DeclareMathSymbol{\varpartialdiff}{\mathord}{letters}{130}
\DeclareMathSymbol{\varvarpi}{\mathord}{letters}{131}
\DeclareMathSymbol{\othervarkappa}{\mathord}{otherletters}{128}
\DeclareMathSymbol{\othervarvarrho}{\mathord}{otherletters}{129}
\DeclareMathSymbol{\othervarvarpi}{\mathord}{otherletters}{131}

%
\DeclareMathDelimiter{(}{\mathopen} {operators}{040}{largesymbols}{161}
\DeclareMathDelimiter{)}{\mathclose}{operators}{041}{largesymbols}{162}
\DeclareMathDelimiter{[}{\mathopen} {operators}{091}{largesymbols}{163}
\DeclareMathDelimiter{]}{\mathclose}{operators}{093}{largesymbols}{164}
\DeclareMathDelimiter{/}{\mathord}{operators}{047}{largesymbols}{177}
\DeclareMathDelimiter{|}{\mathord}{symbols}{106}{largesymbols}{175}
\DeclareMathDelimiter{\llbracket}{\mathopen}{symbols}{153}{largesymbols}{133}
\DeclareMathDelimiter{\rrbracket}{\mathclose}{symbols}{154}{largesymbols}{134}
\def\dblbrackleft{\llbracket\PackageWarningNoLine{fourier}{The command \protect\dblbrackleft\space is deprecated.^^J Use \protect\llbracket\space instead}}
\def\dblbrackright{\rrbracket\PackageWarningNoLine{fourier}{The command \protect\dblbrackright\space is deprecated.^^J Use \protect\rrbracket\space instead}}

%
\expandafter\DeclareMathDelimiter\@backslashchar
                        {\mathord}{symbols}{110}{largesymbols}{178}
\DeclareMathDelimiter{\Vert}
   {\mathord}{symbols}{107}{largesymbols}{176}
\DeclareMathDelimiter{\VERT}
   {\mathord}{symbols}{152}{largesymbols}{147}
\let\|=\Vert
\DeclareMathDelimiter{\vert}
   {\mathord}{symbols}{106}{largesymbols}{175}
    \DeclareMathDelimiter{\lvert}
      {\mathopen}{symbols}{106}{largesymbols}{175}
    \DeclareMathDelimiter{\rvert}
      {\mathclose}{symbols}{106}{largesymbols}{175}
    \DeclareMathDelimiter{\lVert}
      {\mathopen}{symbols}{107}{largesymbols}{176}
    \DeclareMathDelimiter{\rVert}
      {\mathclose}{symbols}{107}{largesymbols}{176}
\DeclareMathDelimiter{\Downarrow}
{\mathrel}{symbols}{043}{largesymbols}{196}
\DeclareMathDelimiter{\backslash}    % for double coset G\backslash H
   {\mathord}{symbols}{110}{largesymbols}{178}
\DeclareMathDelimiter{\rangle}
   {\mathclose}{symbols}{105}{largesymbols}{174}
\DeclareMathDelimiter{\langle}
   {\mathopen}{symbols}{104}{largesymbols}{173}
\DeclareMathDelimiter{\rbrace}
   {\mathclose}{symbols}{103}{largesymbols}{170}
\DeclareMathDelimiter{\lbrace}
   {\mathopen}{symbols}{102}{largesymbols}{169}
\DeclareMathDelimiter{\rceil}
   {\mathclose}{symbols}{101}{largesymbols}{168}
\DeclareMathDelimiter{\lceil}
   {\mathopen}{symbols}{100}{largesymbols}{167}
\DeclareMathDelimiter{\rfloor}
   {\mathclose}{symbols}{99}{largesymbols}{166}
\DeclareMathDelimiter{\lfloor}
   {\mathopen}{symbols}{98}{largesymbols}{165}
%%%%%%


\DeclareMathAccent{\acute}{\mathalpha}{operators}{1}
\DeclareMathAccent{\grave}{\mathalpha}{operators}{0}
\DeclareMathAccent{\ddot}{\mathalpha}{operators}{4}
\DeclareMathAccent{\tilde}{\mathalpha}{operators}{3}
\DeclareMathAccent{\bar}{\mathalpha}{operators}{9}
\DeclareMathAccent{\breve}{\mathalpha}{operators}{8}
\DeclareMathAccent{\check}{\mathalpha}{operators}{7}
\DeclareMathAccent{\hat}{\mathalpha}{operators}{2}
\DeclareMathAccent{\dot}{\mathalpha}{operators}{10}
\DeclareMathAccent{\mathring}{\mathalpha}{operators}{6}
\DeclareMathAccent{\wideparen}{\mathord}{largesymbols}{148}
%%

\DeclareMathAccent{\widearc}{\mathord}{largesymbols}{216}
\DeclareMathAccent{\wideOarc}{\mathord}{largesymbols}{228}
%%
\def\defaultscriptratio{.76}
\def\defaultscriptscriptratio{.6}
\DeclareMathSizes{5}     {6}   {6}  {6}
\DeclareMathSizes{6}     {6}   {6}  {6}
\DeclareMathSizes{7}     {6.8} {6}  {6}
\DeclareMathSizes{8}     {8}   {6.8}{6}
\DeclareMathSizes{9}     {9}   {7.6}{6}
\DeclareMathSizes{10}   {10}   {7.6}{6}
\DeclareMathSizes{10.95}{10.95}{8.3}{6}
\DeclareMathSizes{12}   {12}   {9}  {7}
\DeclareMathSizes{14.4} {14.4} {10} {8}
\DeclareMathSizes{17.28}{17.28}{12} {9}
\DeclareMathSizes{20.74}{20.74}{14.4}{10}
\DeclareMathSizes{24.88}{24.88}{17.28}{12}
\thinmuskip=2mu
\medmuskip=2.5mu plus 1mu minus 2.5mu
\thickmuskip=3.5mu plus 2.5mu
%%
\delimiterfactor850
%%
\DeclareFontFamily{U}{futm}{}
\DeclareFontShape{U}{futm}{m}{n}{
  <-> s * [.92] fourier-bb
  }{}
\DeclareSymbolFont{Ufutm}{U}{futm}{m}{n}
\DeclareSymbolFontAlphabet{\math@bb}{Ufutm}
\AtBeginDocument{\let\mathbb\math@bb %
\DeclareMathSymbol{\iintop}{\mathop}{largesymbols}{206}
  \DeclareMathSymbol{\iiintop}{\mathop}{largesymbols}{208}
  \DeclareMathSymbol{\oiintop}{\mathop}{largesymbols}{210}
  \DeclareMathSymbol{\oiiintop}{\mathop}{largesymbols}{212}
  \DeclareMathSymbol{\slashintop}{\mathop}{largesymbols}{214}
  \@ifpackageloaded{amsmath}{%
    \def\iint{\DOTSI\iintop\ilimits@}
    \def\iiint{\DOTSI\iiintop\ilimits@}
    \def\oiint{\DOTSI\oiintop\ilimits@}
    \def\oiiint{\DOTSI\oiiintop\ilimits@}
    \def\slashint{\DOTSI\slashintop\ilimits@}
  }{%
     \def\iint{\iintop\nolimits}
     \def\iiint{\iiintop\nolimits}
     \def\oiint{\oiintop\nolimits}
     \def\oiiint{\oiiintop\nolimits}
     \def\slashint{\slashintop\nolimits}
  }
    \@ifpackageloaded{amsfonts}{%
     \let\widehat\undefined
     \DeclareMathAccent{\widehat}{\mathord}{largesymbols}{98}
     \let\widetilde\undefined
     \DeclareMathAccent{\widetilde}{\mathord}{largesymbols}{101}
  }{}
  \ifx\overset\@undefined\else
    \newcommand{\widering}[1]{\overset{\smash{\vbox to .2ex{%
    \hbox{$\mathring{}$}}}}{\wideparen{#1}}}
  \fi
%
  \def\accentclass@{0} % I'm unsure whether this is ok
}
%
%
\endinput


